A Survey and Evaluation of Adversarial Attacks for Object Detection

Deep learning models achieve remarkable accuracy in computer vision tasks, yet remain vulnerable to adversarial examples--carefully crafted perturbations to input images that can deceive these models into making confident but incorrect predictions. This vulnerability pose significant risks in high-stakes applications such as autonomous vehicles, security surveillance, and safety-critical inspection systems. While the existing literature extensively covers adversarial attacks in image classification, comprehensive analyses of such attacks on object detection systems remain limited. This paper presents a novel taxonomic framework for categorizing adversarial attacks specific to object detection architectures, synthesizes existing robustness metrics, and provides a comprehensive empirical evaluation of state-of-the-art attack methodologies on popular object detection models, including both traditional detectors and modern detectors with vision-language pretraining. Through rigorous analysis of open-source attack implementations and their effectiveness across diverse detection architectures, we derive key insights into attack characteristics. Furthermore, we delineate critical research gaps and emerging challenges to guide future investigations in securing object detection systems against adversarial threats. Our findings establish a foundation for developing more robust detection models while highlighting the urgent need for standardized evaluation protocols in this rapidly evolving domain.

==> tnnls_sections/related_works.tex <==
\section{Related Works}
\label{sec: related works}

Amongst existing surveys and evaluations, most works targeted image classification \cite{akhtar2018cvsurveythreat, huang2020cvsurvey, ding2020cvsurvey, charkraborty2021cvsurvey, tan2022cvsurvey, wang2022cvsurveyblackbox, croce2020robustbench, tang2021robustart, ren2021advret}. \cite{amirkhani2022surveyav} focused on object detection for the autonomous vehicle application. \cite{mi2023surveyod} surveyed adversarial attacks and defences, but did not survey evaluation procedures and did not provide an evaluation of attacks. A fair comparison of the effectiveness of attack methods based only on published manuscripts is difficult, as works evaluate on different object detection models, use different evaluation datasets (e.g. full public datasets \cite{chow2020tog, chen2022rad} versus subsets \cite{cai2023ensemble, cai2022zqa} or proprietary datasets \cite{xu2020evaluation}), metrics (e.g. mAP \cite{chow2020tog, chen2022rad} versus custom metrics \cite{cai2023ensemble, cai2022zqa}), attack targets (e.g. all classes \cite{chow2020tog} versus only `Person' class \cite{wang2022transpatch, wu2020cloakeccv}) and hyperparameters (e.g. small \cite{cai2022zqa} versus large number of queries \cite{liang2021prfa, wang2022daedalus}). 

There are limited evaluation works on object detection-specific adversarial attacks. Some factors that may have contributed to this include: (1) numerous works did not open-source their code and (2) the open-source code repositories have different dependencies such that they may not support the same set of object detection models. Xu et al. \cite{xu2020evaluation} evaluated six adversarial attacks on their effectiveness, time cost, number of attack iterations and magnitute of image distortion. \cite{hingun2022reap} evaluated how adversarial patches affect the robustness of object detectors on road signs. Both works focused on the white-box setting. \cite{du2022detectsec} and \cite{yang2018cloak} explored attack transferability in the black-box setting, but \cite{du2022detectsec} only tested two object detection-specific attack algorithms, and \cite{yang2018cloak} tested one patch attack algorithm and focused on comparing different patch patterns. A summary is shown in Table \ref{tab: bench_object}. Out of the evaluation works, only \cite{hingun2022reap} is open-sourced. 

\input{tnnls_tables/bench_ob}


==> tnnls_tables/bench_img.tex <==
\begin{table}[htb]

\centering
% \setlength{\tabcolsep}{2pt}
\begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{p{}p{}p{}p{}p{1cm}p{}p{}p{}}
\begin{tabular}{lllllllll}

\toprule[1pt]\midrule[0.3pt]

\textbf{Name} & \multicolumn{ 2}{c}{\textbf{Software}}  & \multicolumn{ 2}{c}{\textbf{Attack Methods}} & \multicolumn{ 4}{c}{\textbf{Robustness Evaluation}} \\ 
\cmidrule(lr){2-3}    
\cmidrule(lr){4-5}
\cmidrule(lr){6-9}    

& \multicolumn{1}{c}{Pytorch} & \multicolumn{1}{c}{Last update} & \multicolumn{1}{c}{Task} & \multicolumn{1}{c}{Knowledge} & \multicolumn{1}{c}{\# Model} & \multicolumn{1}{c}{\# Attack} &  \multicolumn{1}{c}{Metric} &  \multicolumn{1}{c}{Datasets} \\ 

\midrule[0.3pt]

RobustBench & Yes & 2022  & CLF & white/black & 80+ & FGSM, PGD, Auto & CA, RA  & CIFAR, ImageNet \\ 
RobustART & Yes & 2023  & CLF & white/black & 1200+ & FGSM, PGD, Auto & CA, RA  & ImageNet\\ 

% \midrule
% \multirow{ 2}{*}{Image} & Common objects & VOC-2007, VOC-2012, COCO, KITTI\\
%                         & Person & Inria Person, CityPersons, ImageNet$^\dagger$ \\ 
%                         & Traffic sign & Stop Sign, Mapilliary$^\dagger$ \\ \hdashline
% Video                   & Common objects & ImageNet VID \\
% \midrule[0.3pt]
\bottomrule[1pt]
\end{tabular}
\end{adjustbox}

\caption{Adversarial robustness benchmarking evaluations on image classification task. \protect\label{tab: bench_img}}

\end{table}

==> tnnls_tables/bench_toolbox.tex <==
\begin{table*}[htb]

\centering
% \setlength{\tabcolsep}{2pt}
\begin{adjustbox}{max width=0.8\textwidth}
% \begin{tabular}{p{}p{}p{}p{}p{1cm}p{}p{}p{}}
\begin{tabular}{llllllll}

\toprule[1pt]\midrule[0.3pt]

\textbf{Name} & \multicolumn{ 2}{c}{\textbf{Software}}  & \multicolumn{ 2}{c}{\textbf{Applications}} & \multicolumn{ 3}{c}{\textbf{Attack Methods}} \\ 
\cmidrule(lr){2-3}    
\cmidrule(lr){4-5}
\cmidrule(lr){6-8}    

& \multicolumn{1}{c}{Framework} & \multicolumn{1}{c}{Last update} & \multicolumn{1}{c}{Data} & \multicolumn{1}{c}{Task} & \multicolumn{1}{c}{Knowledge} & \multicolumn{1}{c}{Pertubation} &  \multicolumn{1}{c}{OD Attack Methods} \\ 

\midrule[0.3pt]

Foolbox & PyTorch & 2022  & image & CLS & white/black-box & $l_1$ $l_2$ $l_\infty$ & FGSM, PGD \\ 
CleverHans & PyTorch & 2021  & image & CLS & white-box & $l_1$ $l_2$ $l_\infty$ & CW, FGSM, PGD \\ 
AdverTorch & PyTorch & 2022  & image & CLS & white/black-box & $l_1$ $l_2$ $l_\infty$ & CW, FGSM, PGD \\ 
MadryLab & PyTorch & 2021  & image & CLS & white-box & $l_2$ $l_\infty$ & CW, FGSM, PGD \\ 
ART & PyTorch & 2024  & image, audio, video &   CLS, OD & white/black-box, poisoning & $l_1$ $l_2$ $l_\infty$ & FGSM, PGD, DPatch \\ 

% \midrule
% \multirow{ 2}{*}{Image} & Common objects & VOC-2007, VOC-2012, COCO, KITTI\\
%                         & Person & Inria Person, CityPersons, ImageNet$^\dagger$ \\ 
%                         & Traffic sign & Stop Sign, Mapilliary$^\dagger$ \\ \hdashline
% Video                   & Common objects & ImageNet VID \\
% \midrule[0.3pt]
\bottomrule[1pt]
\end{tabular}
\end{adjustbox}

\caption{Open-source adversarial robustness toolbox. \protect\label{tab: bench_toolbox}}

\end{table*}
